Securing Databases from Probabilistic Inference

Databases can leak confidential information when users combine query results with probabilistic data dependencies and prior knowledge. Current research offers mechanisms that either handle a limited class of dependencies or lack tractable enforcement algorithms. We propose a foundation for Database Inference Control based on ProbLog, a probabilistic logic programming language. We leverage this foundation to develop Angerona, a provably secure enforcement mechanism that prevents information leakage in the presence of probabilistic dependencies. We then provide a tractable inference algorithm for a practically relevant fragment of ProbLog. We empirically evaluate Angerona's performance showing that it scales to relevant security-critical problems.

==> atklog_lite.tex <==
\section{AtkLog-Lite}\label{sect:atklog:lite}

\remark{{\bf TODO}
\begin{compactitem}
\item Simplify templates and guarded cycles.
%
\item Write Join-Acyclic rules and Join-Safe paths.
%
\item Running Example from beginning to generated BN!!!!
%
\item Double check whether all examples in Appendix~\ref{app:language:examples} are in \atkloglite{}.
\end{compactitem}
}

%
Exact probabilistic inference in \atklog{} is intractable in general, i.e., it is $\#P$-hard~\cite{koller2009probabilistic}, due to the expressive power of \problog{}, the language used to formalize B-programs.
%
This limits the practical applicability of \atklog{}.



To address this, we present \atkloglite{}, an \atklog{} fragment that (1) is expressive enough to encode realistic probabilistic models, such as those associated with the examples from \S\ref{sect:motivating:example}, and (2) supports efficient probabilistic inference, namely at most in quadratic time in the size of the domain.
%
The key insight behind \atkloglite{} is requiring the \problog{} B-programs to be \emph{acyclic}.
%
This ensures that the \problog{} program can be compiled to an equivalent poly-tree Bayesian Network where inference can be performed efficiently, i.e., in linear time in the network's size~\cite{koller2009probabilistic}.


We now introduce the main ideas behind acyclic \problog{} programs.
%
%In the following, let $\Sigma$ be a database schema, $\mathbf{dom}$ be a finite domain, and $p$ be a $(\Sigma, \mathbf{dom})$-\problog{} program.

\remark{TO DO}

%
%Appendix~\ref{app:atklog:lite:extended} presents the formal definition of acyclic \problog{} programs.
%
%It also presents the encoding of acyclic \problog{} programs together with all the correctness and complexity proofs.




\begin{comment}
\para{Templates}
%
Templates are used to express invariants about all well-founded models associated with a given \problog{} program.
%
In particular, we define three kinds of templates: ordering, disjointness, and uniqueness templates.


A \emph{$\Sigma$-ordering template} is a set of predicate symbols in $\Sigma$ of even arity. 
%
Intuitively, an ordering template indicates those predicates whose transitive closure is a strict partial order.
%
A program $p$ complies with an ordering template ${\cal O}$ iff for all predicate symbols $\mathit{pr} \in {\cal O}$, the relation $\{ (\overline{a}, \overline{b})  \mid |\overline{a}| = | \overline{b}| = \sfrac{|\mathit{pr}|}{2} \wedge  \mathit{pr}(\overline{a}, \overline{b}) \in \bigcup_{f \in A(p)}\mathit{WFM}(\mathit{instance}(p,f))\}$ is a strict partial order.

%
A \emph{$\Sigma$-disjointness template} is a set of pairs of predicate symbols in $\Sigma$ with the same arity. 
%
Intuitively, a disjointness template contains pair of predicate symbols whose associated relations are always disjoint.
%
A program $p$ complies with a disjointness template ${\cal D}$ iff for all $(\mathit{pr},\mathit{pr}') \in {\cal D}$, 
$\{ \overline{a}  \mid  \mathit{pr}(\overline{a}) \in \bigcup_{f \in A(p)} \mathit{WFM}(\mathit{instance}(p,f))\} \cap \{ \overline{a}  \mid  \mathit{pr}'(\overline{a}) \in \bigcup_{f \in A(p)}\mathit{WFM}(\mathit{instance}(p,f))\} = \emptyset$.

%
A \emph{$\Sigma$-uniqueness template} is a function associating to each predicate symbol $\mathit{pr} \in \Sigma$, a set $K \in \mathbb{P}(\{1,\ldots, |\mathit{pr}|\})$.
%
Intuitively, a uniqueness template associates to each predicate symbol a set of primary key constraints.
%
A program $p$ complies with a uniqueness template ${\cal U}$ iff for all $\mathit{pr} \in \Sigma$ and all $\overline{t}, \overline{t}' \in \mathbf{dom}^*$ such that $\mathit{pr}(\overline{t}), \mathit{pr}(\overline{t}') \in \bigcup_{f \in A(p)} \mathit{WFM}(\mathit{instance}(p,f))$, if $\overline{t}(i) = \overline{t}'(i)$ for all $i \in {\cal U}(\mathit{pr})$, then $\overline{t} = \overline{t}'$.

%
Appendix~\ref{app:atklog:lite:extended} presents simple syntactic rules for determining whether a program complies with these templates.


\begin{example}\label{example:template}
Let $p$ be the \problog{} program from Example~\ref{example:atklog:bprogram}.
%
The program complies with the ordering template ${\cal O} = \{\mathit{father}, \mathit{mother}\}$ and with the disjointness template ${\cal D} = \{(\mathit{father}, \mathit{mother})\}$ since the relations defined by $\mathit{father}$ and $\mathit{mother}$ are strict partial orders and are disjoint.
%
It complies also with the uniqueness template ${\cal U} = \{\mathit{patient} \mapsto \{\{1\}\}, \mathit{smokes} \mapsto \{\{1\}\}, \mathit{cancer} \mapsto \{\{1\}\}, \mathit{father} \mapsto \{\{2\}\}, \mathit{mother} \mapsto \{\{2\}\}\}$. For the predicate symbols $\mathit{patient}$, $\mathit{smokes}$, and $\mathit{cancer}$, the primary key constraints are trivially satisfied since the predicates' arity is $1$.
%
For the predicate symbols $\mathit{father}$ and $\mathit{mother}$, the second attribute, i.e., the child, acts as primary key.
\end{example}

\para{Dependency Graphs}
%
The dependency graph of a program $p$, denoted $\mathit{graph}(p)$, is the directed labelled graph $(N,E)$, where $N = \Sigma$ and $E = \{ \mathit{pred}(\mathit{body}(r,i)) \xrightarrow{r,i} \mathit{pred}(\mathit{head}(r)) \mid r \in p \wedge i \in \mathbb{N} \}$.
%
A dependency graph may contain two kinds of cycles:
%
\begin{inparaenum}[(a)]
\item a \emph{type-1 cycle} in $\mathit{graph}(p)$ is a  cycle $\mathit{pr}_1 \xrightarrow{r_1, i_1} \ldots \xrightarrow{r_{n-1}, i_{n-1}} \mathit{pr}_n \xrightarrow{r_n, i_n} \mathit{pr}_1$ in $\mathit{graph}(p)$, and
%
\item a \emph{type-2 cycle} in $\mathit{graph}(p)$ is a pair of distinct paths $(\mathit{pr} \xrightarrow{r_1,i_1} \ldots \xrightarrow{r_n, i_n} \mathit{pr}', \mathit{pr} \xrightarrow{r_1',i_1'} \ldots \xrightarrow{r_m', i_m'} \mathit{pr}')$ in $\mathit{graph}(p)$.
\end{inparaenum}
%

\begin{example}
Figure~\ref{figure:dependency:graph:medical} shows the dependency graph associated with the program from Example~Example~\ref{example:atklog:bprogram}.
%

\end{example}

%\begin{figure}
%\centering
%\begin{tikzpicture}
%	\node[shape=circle, draw=black, minimum width=2.2em, anchor=center] (patient) at (0,0) {$\mathit{patient}$};
%	\node[shape=circle, draw=black, minimum width=2.2em, anchor=center] (father) at ($(Q)+(3,0)$) {$\mathit{father}$};
%	\node[shape=circle, draw=black, minimum width=2.2em, anchor=center] (mother) at ($(Q)+(-3,0)$) {$\mathit{mother}$};
%	\node[shape=circle, draw=black, minimum width=2.2em, anchor=center] (smokes) at ($(Q)+(1.5,1)$) {$\mathit{smokes}$};
%	\node[shape=circle, draw=black, minimum width=2.2em, anchor=center] (cancer) at ($(Q)+(1.5,2.5)$) {$\mathit{cancer}$};
%	
%	\path [->] 	(patient) edge node[pos=0.5, below, sloped] {{\small $r_9,2$}} (A);
%	\path [->, dashed] 	(Q) edge node[pos=0.5, below, sloped, ] {{\small $r_9,1$}} (A);
%	\path [->, dashed] 	(Q) edge node[pos=0.5, below, sloped] {{\small $r_{10},1$}} (B);
%	\path [->] 	(R) edge node[pos=0.5, below, sloped] {{\small $r_{10},2$}} (B);
%	\path [->, dashed] 	(A) edge node[pos=0.5, above, sloped] {{\small $r_{11},1$}} (B);
%	\path [->] 	(P) edge node[pos=0.5, above, sloped] {{\small $r_6,2$}} (O);
%	\path [->] 	(Q) edge node[pos=0.5, above, sloped] {{\small $r_6,1$}} (O);
%	\path [->] 	(O) edge node[pos=0.5, above, sloped] {{\small $r_7,1$}} (E);
%	\path [->, densely dotted] 	(G) edge[bend right] node[pos=0.5, above, sloped] {{\small $r_7,2$}} (E);
%	\path [->, densely dotted] 	(E) edge[bend right] node[pos=0.5, above, sloped] {{\small $r_8,1$}} (G);
%	\path [->] 	(F) edge node[pos=0.5, above, sloped] {{\small $r_{13},1$}} (G);
%	\path [->] 	(V) edge node[pos=0.5, below, sloped] {{\small $r_7,3$}} (E);
%	\path [->] 	(P) edge node[pos=0.5, above, sloped] {{\small $r_{15},2$}} (D);
%	\path [->] 	(R) edge node[pos=0.5, above, sloped] {{\small $r_{16},2$}} (C);
%	\path [->, densely dotted] 	(D) edge[bend right] node[pos=0.5, above, sloped] {{\small $r_{15},1$}} (C);
%	\path [->, densely dotted] 	(C) edge[bend right] node[pos=0.5, above, sloped] {{\small $r_{16},1$}} (D);
%\end{tikzpicture}
%\caption{Dependency graph for the program in Example~\ref{example:acyclic:rule:graph}. 
%Type-1 cycles are depicted using dotted edges, whereas type-2 cycles are depicted using dahsed edges.}\label{figure:acyclic:dependency:graph}
%\end{figure}

\para{Guarded Cycles}
%
Guarded cycles are a key concept for acyclic \problog{} programs, as they are one of the preconditions for encoding the program as a poly-tree Bayesian Network.
%
%Let ${\cal O}$ be an ordering template, ${\cal D}$ be a disjointness template, and $p$ be a \problog{} program that complies with ${\cal O}$ and ${\cal D}$.
%
A type-1 cycle $\mathit{pr}_1 \xrightarrow{r_1, i_1} \ldots \xrightarrow{r_{n-1}, i_{n-1}} \mathit{pr}_n \xrightarrow{r_n, i_n} \mathit{pr}_1$ in $\mathit{graph}(p)$ is \textit{${\cal O}$-guarded} iff there is a predicate $\mathit{pr} \in {\cal O}$, a list of integers $\overline{v} = (v_1, \ldots, v_{\sfrac{|\mathit{pr}|}{2}})$, and a non-empty $K \subseteq \{ k \in \mathbb{N} \mid 1 \leq k \leq n\}$ such that%
\begin{compactitem}
\item for all $j \in \{1, \ldots, n\} \setminus K$ and $1 \leq w \leq \sfrac{|\mathit{pr}|}{2}$, $\mathit{args}(\mathit{head}(r_j))(v_w) = \mathit{args}(\mathit{body}(r_j,i_j))(v_w)$, and
%
\item for all $k \in K$ and $1 \leq w \leq \sfrac{|\mathit{pr}|}{2}$, there is literal $l \in \mathit{body}(r_k)$ such that $\mathit{pred}(l) = \mathit{pr}$, $\mathit{args}(l)(w) = \mathit{args}(\mathit{head}(r_j))(v_l)$, and 
$\mathit{args}(l)(\sfrac{|\mathit{pr}|}{2}+w) = \mathit{args}(\mathit{body}(r_j,i_j))(v_w)$.
\end{compactitem}
%
A type-1 cycle $\mathit{pr}_1 \xrightarrow{r_1, i_1} \ldots \xrightarrow{r_{n-1}, i_{n-1}} \mathit{pr}_n \xrightarrow{r_n, i_n} \mathit{pr}_1$ in $\mathit{graph}(p)$ is \textit{${\cal D}$-guarded} iff there is a pair of predicates $(\mathit{pr},\mathit{pr}') \in {\cal D}$, a list of integers $\overline{v} = (v_1, \ldots, v_{{|\mathit{pr}|}})$, and values $1 \leq k,k' \leq n$ such that:
\begin{compactitem}
\item for all $1 \leq j \leq n$ and $1 \leq w \leq |\mathit{pr}|$, $\mathit{args}(\mathit{head}(r_j))(v_w) = \mathit{args}(\mathit{body}(r_j,i_j))(v_w)$, and
%
\item there are literals $l \in \mathit{body}(r_k)$ and $l' \in \mathit{body}(r_{k'})$ such that $\mathit{pred}(l) = \mathit{pr}$, $\mathit{pred}(l') = \mathit{pr}'$, and for all $1 \leq w \leq |\mathit{pr}|$,  $\mathit{args}(\mathit{head}(r_k))(v_w) = \mathit{args}(l)(w)$ and $\mathit{args}(\mathit{head}(r_{k'}))(v_w) = \mathit{args}(l')(w)$.
\end{compactitem}
%
Finally, a type-2 cycle $(\mathit{pr} \xrightarrow{r_1,i_1} \ldots \xrightarrow{r_n, i_n} \mathit{pr}', \mathit{pr} \xrightarrow{r_1',i_1'} \ldots \xrightarrow{r_m', i_m'} \mathit{pr}')$ in $\mathit{graph}(p)$ is \textit{${\cal D}$-guarded} iff there is a pair of predicates $(\mathit{pr},\mathit{pr}') \in {\cal D}$, a list of integers $\overline{v} = (v_1, \ldots, v_{{|\mathit{pr}|}})$, and values $1 \leq k \leq n$ and $1 \leq k' \leq m$ such that:
\begin{compactitem}
\item for all $1 \leq j \leq n$ and $1 \leq w \leq |\mathit{pr}|$, $\mathit{args}(\mathit{head}(r_j))(v_w) = \mathit{args}(\mathit{body}(r_j,i_j))(v_w)$, 
%
\item for all $1 \leq j \leq n'$ and $1 \leq w \leq |\mathit{pr}|$, $\mathit{args}(\mathit{head}(r_j'))(v_w) = \mathit{args}(\mathit{body}(r_j',i_j'))(v_w)$, and
%
\item there are literals $l \in \mathit{body}(r_k)$ and $l' \in \mathit{body}(r_{k'})$ such that $(\mathit{pred}(l),\mathit{pred}(l')) = (\mathit{pr}, \mathit{pr}')$ and for all $1 \leq w \leq |\mathit{pr}|$,  $\mathit{args}(\mathit{head}(r_k))(v_w) = \mathit{args}(l)(w)$ and $\mathit{args}(\mathit{head}(r_{k'}'))(v_w) = \mathit{args}(l')(w)$.
\end{compactitem}





\para{Join Trees, Join-Acyclic Rules, and Join-Safe Paths}
%
A \emph{join tree for  a rule $r$} is a labelled tree $(N,E)$ such that
%
(1) $N \subseteq \mathit{body}(r)$,
%
(2) for all $n \xrightarrow{L} n' \in E$, $n, n' \in \mathit{body}^+(r)$, $L = \mathit{vars}(n) \cap \mathit{vars}(n')$, and $L \neq \emptyset$.
%
We say that a join tree $(N,E)$ \emph{covers} a literal $l$ iff $l \in N$.


Given a join tree $J=(N,E)$ and a node $n \in N$, the \emph{support of $n$}, denoted $\mathit{support}(n)$, is the set $\mathit{vars}(\mathit{head}(r)) \cup \{ x \mid (x = c) \in \mathit{cstr}(r) \wedge c \in \mathbf{dom} \} \cup \{ \mathit{vars}(n')  \mid p = \mathit{root}(J) \to \ldots \to n \wedge p \in \mathit{paths}(J) \wedge n'\to n'' \in p\}$, where $\mathit{paths}(J)$ is the set of all paths in the join tree and $\mathit{root}(J)$ is $J$'s root.
%
We say that a join tree $J=(N,E)$ is \emph{strongly connected for ${\cal U}$} iff
%
for all $l \in N$, the following conditions hold:
%
\begin{compactitem}
\item If $l$ is a positive literal, then there is a set $K \subseteq \{ i \mid \overline{x} = \mathit{vars}(l) \wedge \overline{x}(i) \in \mathit{support}(l) \}$ such that $K \in {\cal U}(\mathit{pred}(l))$.
%
\item If $l$ is a negative literal, then $\mathit{vars}(l) \subseteq \mathit{support}(l)$.
\end{compactitem}

%
We say that a join tree $(N,E)$ is \emph{weakly connected for ${\cal U}$} iff
%
for all $l(\overline{x}) \xrightarrow{L} l'(\overline{x}') \in E$, there are $K \subseteq \{ i \mid \overline{x}(i) \in L \}$ and $K' \subseteq \{ i \mid \overline{x}'(i) \in L \}$  such that $K \in {\cal U}(\mathit{pred}(l))$ and $K' \in {\cal U}(\mathit{pred}(l'))$.





%
Given a rule $r$, a set of literals $L$, and a uniqueness template ${\cal U}$, we say that a literal $l \in \mathit{body}(r)$ is \textit{$(r,{\cal U},L)$-strictly guarded} iff 
%
(1) $\mathit{vars}(l) \subseteq \bigcup_{l' \in  L\cap\mathit{body}^+(r)} \mathit{vars}(l') \cup \{x \mid (x = c) \in \mathit{cstr}(r) \wedge c \in \mathbf{dom}\}$, and
%
(2) there is a positive literal $a(\overline{x}) \in L\cap\mathit{body}^+(r)$ and a $K \in {\cal U}(a)$ such that $\{ \overline{x}(i) \mid i \in K \} \subseteq \mathit{vars}(l)$.
%
A rule $r$ is \emph{weakly connected for ${\cal U}$} iff 
%
there exists a join tree $J = (N,E)$ such that (a) $J$ is weakly connected for ${\cal U}$, (b) $N \subseteq \mathit{body}^+(r)$, and (c) all literals in $\mathit{body}(r) \setminus N$ are $(r,{\cal U}, N)$-strictly guarded.

%
A rule $r$ is \emph{strongly connected for ${\cal U}$} iff there exist join trees $J_1, \ldots, J_n$ such that (a) the trees cover all literals in $\mathit{body}(r)$, and (b) for each $1 \leq i \leq n$,  $J_i$ is strongly connected for ${\cal U}$.
%
Furthermore, a rule $r$ is \emph{join-acyclic for ${\cal U}$} iff $r$ is strongly or weakly connected for ${\cal U}$.
%
Finally, a path $\mathit{pr}_1 \xrightarrow{r_1, i_1} \ldots \xrightarrow{r_{n-1}, i_{n-1}} \mathit{pr}_n$ in $\mathit{graph}(p)$ is \emph{join-safe for ${\cal U}$} iff 
%
\begin{inparaenum}[(1)]
\item all rules $r_i$ are strongly connected for ${\cal U}$,
%
\item all rules $r_i$ are weakly connected for ${\cal U}$, or
%
there is a $1 \leq j < n$ such that all $r_i$, where $1 \leq i \leq j$, are weakly connected for ${\cal U}$ and all $r_k$, where $j < k < n$, are strongly connected for ${\cal U}$.
\end{inparaenum}



\para{Acyclic Programs}
%
A $(\Sigma, \mathbf{dom})$-program $p$ is \emph{acyclic} iff there are a $\Sigma$-ordering template ${\cal O}$, a $\Sigma$-disjointness template ${\cal D}$, and a $\Sigma$-uniqueness template ${\cal U}$ such that%
\begin{inparaenum}[(1)]
\item $p$ complies with ${\cal O}$, ${\cal D}$, and ${\cal U}$,
%
\item all rules in $p$ are join-acyclic for ${\cal U}$,
%
\item all paths in $\mathit{graph}(p)$ are join-safe,
%
\item for all rules $r \in p$ and all negative literals $l \in \mathit{body}^-(r)$, $\mathit{vars}(l) \subseteq \bigcup_{l \in \mathit{body}^+(r)} \mathit{vars}(l)$,
%
\item all type-1 cycles in $\mathit{graph}(p)$ are either ${\cal O}$-guarded or ${\cal D}$-guarded, and 
%
\item all type-2 cycles in $\mathit{graph}(p)$ are ${\cal D}$-guarded.
\end{inparaenum}

\end{comment}

\para{Inference}
%
Exact inference for an acyclic \problog{} program $p$ can be performed in three steps.
%
First, we compute the \emph{relaxed grounding of $p$}, a sound over-approximation of  the ground version of all possible $p$-grounded instances.
%
Afterwards, we use the relaxed grounding of $p$ to construct the associated Bayesian Network $\mathit{BN}$.
%
Finally, we perform the inference on $\mathit{BN}$ using standard inference algorithms for poly-tree Bayesian Networks~\cite{koller2009probabilistic}.
%
Additional details about the inference decision procedure and the encoding as Bayesian Network, as well correctness and complexity proofs can be found in Appendix~\ref{app:atklog:lite:extended}.

Here, we report the following theorem on the data complexity (i.e., in the size of $\mathbf{dom}$) of the inference task:

\begin{theorem}
The data complexity of inference for acyclic \problog{} programs is \textsc{Ptime}. 
\end{theorem} 

\begin{proofsketch}
The relaxed grounding of $p$ can be computed in linear time in terms of data complexity ($O(|\mathbf{dom}|^k)$).
%
The encoding can be computed in quadratic time ($O(|\mathbf{dom}|^{2k})$) and its size is linear in $O(|\mathbf{dom}^k|)$.
%
Finally, inference for poly-tree Bayesian Networks can be performed in linear time in the network's size~\cite{koller2009probabilistic}.
\end{proofsketch}

